Local Supersymmetry Enhancement and Black Hole Microstates

In string theory, black holes can be made from brane systems that are partially delocalized in string theory's extra dimensions. It is expected that they correspond to an ensemble of pure, horizonless microstates sourced by localized versions of this brane system. This thesis aims at studying the relationship between supersymmetric black holes and their microstates. In particular, we apply a concept called local supersymmetry enhancement to 1/4-BPS and 1/8-BPS systems that correspond to two-, three-, and four-charge black holes. This concept locally increases the number of preserved supercharges to 16 by adding dipole charges to the system. These bound states are then expected to be horizonless and describe the microstates of the black hole. First, we list all dipole charges for 1/4-BPS systems in Type II string theory. Then, we apply these to generate two structures to enhance 1/8-BPS systems, one with exclusively internal dipole charges and the other with a non-trivial shape in the non-compact dimensions. Thus, we identify the dipole charges for the microstates of various supersymmetric black holes, including new internal dipole charges for the D1-D5-P black hole and external ones for the D2-D2-D2-D6 black hole. These dipole charges reveal the local structure of the black hole's microstates and will be used in the construction of the corresponding supergravity solutions.

==> TikzDrawings/CommutationRelations/3ChargeGlueCommutationRules.tex <==
\tikzsetnextfilename{3ChargeGlueCommutationRules}
\begin{tikzpicture}
    \node at (0,0) (P1) [draw, circle, minimum size = 1.5cm] {$P_1$};
    \node at (5,0) (P2) [draw, circle, minimum size = 1.5cm] {$P_2$};
    \node at (2.5,-4.3) (P3) [draw, circle, minimum size = 1.5cm] {$P_3$};

    \draw (P1) -- (P2) 
        node [near start, above] (Q1) {$Q_1$} % add sloped for slanted text
        node [near end, above] (Q2) {$Q_2$};
    \draw (P1) -- (P3) 
        node [near start, left] (Q3) {$Q_3$} 
        node [near end, left] (Q4) {$Q_4$};
    
    \draw [AnticommutingLine] (Q1) -- (Q3);
    \draw [CommutingLine] (Q1) -- (Q4);
    \draw [CommutingLine] (Q2) -- (Q3);
    \draw [AnticommutingLine] (Q2) -- (Q4);
\end{tikzpicture}

==> TikzDrawings/CommutationRelations/AllCommuting.tex <==
\tikzsetnextfilename{AllCommuting}
\begin{tikzpicture}
    \node at (0,0) (P1) [draw, circle, minimum size = 1.5cm] {$P_1$};
    \node at (4,0) (P2) [draw, circle, minimum size = 1.5cm] {$P_2$};
    \node at (0,-4) (Q1) [draw, circle, minimum size = 1.5cm] {$Q_1$};
    \node at (4,-4) (Q2) [draw, circle, minimum size = 1.5cm] {$Q_2$};

    \draw [CommutingLine] (P1) -- (P2);
    \draw [CommutingLine] (Q1) -- (Q2);
    \draw [CommutingLine] (P1) -- (Q1);
    \draw [CommutingLine] (P1) -- (Q2);
    \draw [CommutingLine] (P2) -- (Q1);
    \draw [CommutingLine] (P2) -- (Q2);
\end{tikzpicture}

==> TikzDrawings/CommutationRelations/LSECommuting.tex <==
\tikzsetnextfilename{LSECommuting}
\begin{tikzpicture}
    \node at (0,0) (P1) [draw, circle, minimum size = 1.5cm] {$P_1$};
    \node at (4,0) (P2) [draw, circle, minimum size = 1.5cm] {$P_2$};
    \node at (0,-4) (Q1) [draw, circle, minimum size = 1.5cm] {$Q_1$};
    \node at (4,-4) (Q2) [draw, circle, minimum size = 1.5cm] {$Q_2$};

    \draw [CommutingLine] (P1) -- (P2);
    \draw [CommutingLine] (Q1) -- (Q2);
    \draw [AnticommutingLine] (P1) -- (Q1);
    \draw [AnticommutingLine] (P1) -- (Q2);
    \draw [AnticommutingLine] (P2) -- (Q1);
    \draw [AnticommutingLine] (P2) -- (Q2);
\end{tikzpicture}

==> TikzDrawings/DualityMaps/DualityMapNonStandard.tex <==
\tikzsetnextfilename{DualityMapNonStandard}
\begin{tikzpicture}
    % Dp Dq scope
    \begin{scope}[node distance = 3cm and 4cm]
        % nodes Dp Dq (1)
        \node (D1D9) [IIB, on grid] {$\D{1} \parallel \D{9}$ (1)};
        \node (D2D8) [IIA, on grid, right = of D1D9] {$\D{2} \perp \D{8}$ (1)};
        \node (D3D7) [IIB, on grid, right = of D2D8] {$\D{3} \perp \D{7}$ (1)};
        \node (D4D6) [IIA, on grid, right = of D3D7] {$\D{4} \perp \D{6}$ (1)};
        \node (D5D5) [IIB, on grid, right = of D4D6] {$\D{5} \perp \D{5}$ (1)};
        % arrows between Dp Dq (1)
        \foreach \x in {1,...,4}
        {
            \pgfmathtruncatemacro{\y}{10 - \x}
            \pgfmathtruncatemacro{\u}{\x + 1}
            \pgfmathtruncatemacro{\v}{\y - 1}
            \draw [TDuality] ([yshift=.1cm]D\x D\y.east) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} ([yshift=.1cm]D\u D\v.west);
            \draw [TDuality] ([yshift=-.1cm]D\u D\v.west) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} ([yshift=-.1cm]D\x D\y.east);
        }
        
        % nodes Dp Dq (0)
        \node (D0D8) [IIA, on grid, below = of D1D9] {$\D{0} \parallel \D{8}$ (0)};
        \node (D1D7) [IIB, on grid, right = of D0D8] {$\D{1} \perp \D{7}$ (0)};
        \node (D2D6) [IIA, on grid, right = of D1D7] {$\D{2} \perp \D{6}$ (0)};
        \node (D3D5) [IIB, on grid, right = of D2D6] {$\D{3} \perp \D{5}$ (0)};
        \node (D4D4) [IIA, on grid, right = of D3D5] {$\D{4} \perp \D{4}$ (0)};
        % arrows between Dp Dq (0)
        \foreach \x in {0,...,3}
        {
            \pgfmathtruncatemacro{\y}{8 - \x}
            \pgfmathtruncatemacro{\u}{\x + 1}
            \pgfmathtruncatemacro{\v}{\y - 1}
            \draw [TDuality] ([yshift=.1cm]D\x D\y.east) to [bend left = 7] node[anchor=south] {$T_{\dashv}$} ([yshift=.1cm]D\u D\v.west);
            \draw [TDuality] ([yshift=-.1cm]D\u D\v.west) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} ([yshift=-.1cm]D\x D\y.east);
        }

        % arrows between Dp Dq (1) and Dp Dq (0)
        \foreach \x in {1,...,5}
        {
            \pgfmathtruncatemacro{\y}{10 - \x}
            \pgfmathtruncatemacro{\u}{\x - 1}
            \pgfmathtruncatemacro{\v}{\y - 1}
            \draw [TDuality] ([xshift=.1cm]D\x D\y.south) to [bend left = 7] node[anchor=west] {$T_{\parallel}$} ([xshift=.1cm]D\u D\v.north);
            \draw [TDuality] ([xshift=-.1cm]D\u D\v.north) to [bend left = 7] node[anchor=east] {$T_{\perp}$} ([xshift=-.1cm]D\x D\y.south);
        }
    \end{scope}

    
    % Dp KKM/NS5/KKM* scope
    \begin{scope}[node distance = 3cm and 5cm, yshift = -7cm]
        % nodes Dp KKM 
        \node (D2KKM) [IIA, on grid] {$\D{2} \perp \KKM$ (0)};
        \node (D3KKM) [IIB, on grid, below = of D2KKM] {$\D{3} \perp \KKM$ (1)};
        \node (D4KKM) [IIA, on grid, below = of D3KKM] {$\D{4} \perp \KKM$ (2)};
        \node (D5KKM) [IIB, on grid, below = of D4KKM] {$\D{5} \perp \KKM$ (3)};
        \node (D6KKM) [IIA, on grid, below = of D5KKM] {$\D{6} \perp \KKM$ (4)};
        \node (D7KKM) [IIB, on grid, below = of D6KKM] {$\D{7} \parallel \KKM$ (5)};
        % arrows between Dp KKM and Dp+1 KKM 
        \foreach \x in {2,...,6}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([xshift=.1cm]D\x KKM.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]D\y KKM.north);
            \draw [TDuality] ([xshift=-.1cm]D\y KKM.north) to [bend left = 7] node[anchor=east] {$T_{\parallel}$} ([xshift=-.1cm]D\x KKM.south);
        }

        % nodes Dp NS5
        \node (D3NS5) [IIB, on grid, right = of D2KKM] {$\D{3} \perp \NS$ (0)};
        \node (D4NS5) [IIA, on grid, below = of D3NS5] {$\D{4} \perp \NS$ (1)};
        \node (D5NS5) [IIB, on grid, below = of D4NS5] {$\D{5} \perp \NS$ (2)};
        \node (D6NS5) [IIA, on grid, below = of D5NS5] {$\D{6} \perp \NS$ (3)};
        \node (D7NS5) [IIB, on grid, below = of D6NS5] {$\D{7} \perp \NS$ (4)};
        \node (D8NS5) [IIA, on grid, below = of D7NS5] {$\D{8} \parallel \NS$ (5)};
        % arrows between Dp NS5 and Dp+1 NS5
        \foreach \x in {3,...,7}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([xshift=.1cm]D\x NS5.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]D\y NS5.north);
            \draw [TDuality] ([xshift=-.1cm]D\y NS5.north) to [bend left = 7] node[anchor=east] {$T_{\parallel}$} ([xshift=-.1cm]D\x NS5.south);
        }
        % arrows between Dp KKM and Dp+1 NS5
        \foreach \x in {2,...,7}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([yshift=.1cm]D\x KKM.east) to [bend left = 7] node[anchor=south] {$T_{\dashv*}$} ([yshift=.1cm]D\y NS5.west);
            \draw [TDuality] ([yshift=-.1cm]D\y NS5.west) to [bend left = 7] node[anchor=north] {$T_{\vdash}$} ([yshift=-.1cm]D\x KKM.east);
        }
        
        
        % nodes Dp KKM *
        \node (D4KKM*) [IIA, on grid, right = of D3NS5] {$\D{4} \perp \KKM$ (0)*};
        \node (D5KKM*) [IIB, on grid, below = of D4KKM*] {$\D{5} \perp \KKM$ (1)*};
        \node (D6KKM*) [IIA, on grid, below = of D5KKM*] {$\D{6} \perp \KKM$ (2)*};
        \node (D7KKM*) [IIB, on grid, below = of D6KKM*] {$\D{7} \perp \KKM$ (3)*};
        \node (D8KKM*) [IIA, on grid, below = of D7KKM*] {$\D{8} \perp \KKM$ (4)*};
        \node (D9KKM*) [IIB, on grid, below = of D8KKM*] {$\D{9} \parallel \KKM$ (5)*};
        % arrows between Dp KKM and Dp+1 KKM
        \foreach \x in {4,...,8}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([xshift=.1cm]D\x KKM*.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]D\y KKM*.north);
            \draw [TDuality] ([xshift=-.1cm]D\y KKM*.north) to [bend left = 7] node[anchor=east] {$T_{\parallel}$} ([xshift=-.1cm]D\x KKM*.south);
        }
        % arrows between Dp KKM and Dp+1 NS5
        \foreach \x in {3,...,8}
        {
            \pgfmathtruncatemacro{\y}{\x + 1}
            \draw [TDuality] ([yshift=.1cm]D\x NS5.east) to [bend left = 7] node[anchor=south] {$T_{\perp}$} ([yshift=.1cm]D\y KKM*.west);
            \draw [TDuality] ([yshift=-.1cm]D\y KKM*.west) to [bend left = 7] node[anchor=north] {$T_{\dashv*}$} ([yshift=-.1cm]D\x NS5.east);
        }
    \end{scope}


    % NS5/KKM (1) scope
    \begin{scope}[node distance = 3cm and 5cm, xshift=16cm, yshift = -7cm]
        % nodes P/F1 NS5/KKM
        \node (NS5NS5) [IIAB, on grid] {$\NS \perp \NS$ (1)};
        \node (NS5KKM*) [IIAB, on grid, below = of NS5NS5] {$\NS \perp \KKM$ (1)*};
        \node (KKMKKM**) [IIAB, on grid, below = of NS5KKM*] {$\KKM \perp \KKM$ (1)**};
        % arrows between P Dp and P Dp+1
        \draw [TDuality] ([xshift=.1cm]NS5NS5.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]NS5KKM*.north);
        \draw [TDuality] ([xshift=-.1cm]NS5KKM*.north) to [bend left = 7] node[anchor=east] {$T_{\parallel*}$} ([xshift=-.1cm]NS5NS5.south);
        \draw [TDuality] ([xshift=.1cm]NS5KKM*.south) to [bend left = 7] node[anchor=west] {$T_{\vdash}$} ([xshift=.1cm]KKMKKM**.north);
        \draw [TDuality] ([xshift=-.1cm]KKMKKM**.north) to [bend left = 7] node[anchor=east] {$T_{*\parallel}$} ([xshift=-.1cm]NS5KKM*.south);
        \draw [TDuality] ([xshift=-.7cm]KKMKKM**.north) to [bend left = 30] node[anchor=east] {$T_{\parallel*,\leftrightarrow}$} ([xshift=-.7cm]NS5KKM*.south);
    \end{scope}


    % NS5/KKM (3) scope
    \begin{scope}[node distance = 3cm and 5cm, xshift=16cm, yshift = -16cm]
        % nodes P/F1 NS5/KKM
        \node (NS5KKM) [IIAB, on grid,] {$\NS \perp \KKM$ (3)};
        \node (KKMKKM*) [IIAB, on grid, below = of NS5KKM] {$\KKM \perp \KKM$ (3)*};
        % arrows between P Dp and P Dp+1
        \draw [TDuality] (NS5KKM) to [out=20, in=340, loop] node[anchor=south west] {$T_{\dashv*,\leftrightarrow}$} ();
        \draw [TDuality] ([xshift=.1cm]NS5KKM.south) to [bend left = 7] node[anchor=west] {$T_{\dashv}$} ([xshift=.1cm]KKMKKM*.north);
        \draw [TDuality] ([xshift=-.1cm]KKMKKM*.north) to [bend left = 7] node[anchor=east] {$T_{*\parallel}$} ([xshift=-.1cm]NS5KKM.south);
    \end{scope}

    
    % S duality arrows
    \begin{scope}
        \draw [SDuality] (D5KKM*) to [bend left = 20] node[anchor=south] {$S$} (NS5KKM*);
        \draw [SDuality] (D3NS5) to [bend left = 20] node[anchor=north west] {$S$} (D3D5);
        \draw [SDuality] (D5D5.east) to [bend left = 20] node[anchor=west] {$S$} (NS5NS5.east);
        \draw [SDuality] (D5KKM) to [bend left = 15] node[anchor=south] {$S$} (NS5KKM);
        
        \draw [SDuality] (D3KKM) to [loop left] node[anchor=east] {$S$} ();
        \draw [SDuality] (D5NS5) to [out=30, in=50, loop] node[anchor=south west] {$S_{\leftrightarrow}$} ();
        \draw [SDuality] (KKMKKM**) to [loop below] node[anchor=north] {$S$} ();
    \end{scope}
\end{tikzpicture}


==> TikzDrawings/LuninMathurPath.tex <==
\tikzsetnextfilename{Lunin-Mathur-Path}
\begin{tikzpicture}[node distance = 3cm and 6cm]

    \node (PF1) [IIB, on grid, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\W[y] \parallel \F[y]$ (1) \nodepart{second} 
        $\W[1] \parallel \F[1]$ \\
        $\W[2] \parallel \F[2]$ \\
        $\W[4] \parallel \F[4]$ \\
        $\W[9] \parallel \F[9]$ 
    };


    
    \node (PNS5) [IIB, on grid, right = of PF1, yshift = 2cm, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\W[y] \parallel \NS[y1234]$ (1) \nodepart{second} 
        $\D[1]{1} \perp \D[234]{3}$ \\
        $\D[2]{1} \perp \D[134]{3}$ \\
        $\D[4]{1} \perp \D[123]{3}$ \\
        $\W[9] \parallel \NS[12349]$ 
    };
    \node (placeholder) [on grid, right = of PNS5]{};
    \node (D1D5) [IIB, on grid, right = of placeholder, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\D[y]{1} \parallel \D[y1234]{5}$ (1) \nodepart{second} 
        $\F[y] \parallel \NS[y1234]$ \\
        $\D[y12]{3} \perp \D[y34]{3}$ \\
        $\D[y14]{3} \perp \D[y23]{3}$ \\
        $\W[9] \parallel \KKM[12349;y]$ 
    };

    \draw [TDuality,->] ([yshift=0.5cm]PF1.east) to node[anchor=south, sloped] {$S, T_{1,2,3,4},S$} (PNS5.west);
    \draw [TDuality,->] (PNS5.east) to node[anchor=south] {$T_{y,1},S$} (D1D5.west);



    \node (F1D1) [IIB, on grid, right = of PF1, yshift = -2cm, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\F[y] \perp \D[1]{1}$ (0) \nodepart{second} 
        $\F[1] \perp \D[y]{1}$ \\
        $\W[2] \parallel \D[y12]{3}$ \\
        $\W[4] \parallel \D[y14]{3}$ \\
        $\W[9] \parallel \D[y19]{3}$ 
    };
    \node (D1D3) [IIB, on grid, right = of F1D1, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\D[y]{1} \perp \D[123]{3}$ (0) \nodepart{second} 
        $\D[1]{1} \perp \D[y23]{3}$ \\
        $\D[2]{1} \perp \D[y13]{3}$ \\
        $\W[4] \parallel \NS[y1234]$ \\
        $\W[9] \parallel \NS[y1239]$ 
    };
    \node (D1D52) [IIB, on grid, right = of D1D3, rectangle split, rectangle split parts=2, draw, align=center] 
    {$\D[y]{1} \parallel \D[y1234]{5}$ (1) \nodepart{second} 
        $\D[y14]{3} \perp \D[y23]{3}$ \\
        $\D[y24]{3} \perp \D[y13]{3}$ \\
        $\F[y] \parallel \NS[y1234]$ \\
        $\W[9] \parallel \KKM[12349;y]$ 
    };

    \draw [TDuality,->] ([yshift=-0.5cm]PF1.east) to node[anchor=south, sloped] {$S, T_{y,1}$} (F1D1.west);
    \draw [TDuality,->] (F1D1.east) to node[anchor=south] {$T_{2,3}, S$} (D1D3.west);
    \draw [TDuality,->] (D1D3.east) to node[anchor=south] {$T_{y,4}, (y \leftrightarrow 4)$} (D1D52.west);

    \draw [SDuality] (F1D1) to [loop below] node[anchor=north] {$S_{\leftrightarrow}$} ();
    
\end{tikzpicture}

==> TikzDrawings/TetradAnsatz.tex <==
\tikzsetnextfilename{4ChargeConfiguration}
\begin{tikzpicture}
    \node at (0,0) (P1) [draw, circle, minimum size = 1.0cm] {$P_1$};
    \node at (5,0) (P2) [draw, circle, minimum size = 1.0cm] {$P_2$};
    \node at (2.5,-2.3) (P3) [draw, circle, minimum size = 1.0cm] {$P_3$};
    \node at (2.5,3) (P4) [draw, circle, minimum size = 1.0cm] {$P_4$};

    \draw[black!50] (P1) -- (P2) 
        node [near start, below] (Q1) {$Q_1$} % add sloped for slanted text
        node [near end, below] (Q2) {$Q_2$};
    \draw (P1) -- (P3) 
        node [near start, left] (Q3) {$Q_3$} 
        node [near end, left] (Q4) {$Q_4$};
    \draw (P2) -- (P3) 
        node [near start, right] (Q5) {$Q_5$} 
        node [near end, right] (Q6) {$Q_6$};
    \draw (P1) -- (P4) 
        node [near start, left] (Q7) {$Q_7$} 
        node [near end, left] (Q8) {$Q_8$};
    \draw (P2) -- (P4) 
        node [near start, right] (Q9) {$Q_9$} 
        node [near end, right] (Q10) {$Q_{10}$};
    \draw (P3) -- (P4) 
        node [near start, right] (Q11) {$Q_{11}$} 
        node [near end, right] (Q12) {$Q_{12}$};
\end{tikzpicture}
